Soft labelling for semantic segmentation: Bringing coherence to label down-sampling

In semantic segmentation, training data down-sampling is commonly performed due to limited resources, the need to adapt image size to the model input, or improve data augmentation. This down-sampling typically employs different strategies for the image data and the annotated labels. Such discrepancy leads to mismatches between the down-sampled color and label images. Hence, the training performance significantly decreases as the down-sampling factor increases. In this paper, we bring together the down-sampling strategies for the image data and the training labels. To that aim, we propose a novel framework for label down-sampling via soft-labeling that better conserves label information after down-sampling. Therefore, fully aligning soft-labels with image data to keep the distribution of the sampled pixels. This proposal also produces reliable annotations for under-represented semantic classes. Altogether, it allows training competitive models at lower resolutions. Experiments show that the proposal outperforms other down-sampling strategies. Moreover, state-of-the-art performance is achieved for reference benchmarks, but employing significantly less computational resources than foremost approaches. This proposal enables competitive research for semantic segmentation under resource constraints.

==> rebut <==


REBUTTAL STOPS HERE!!


\toreviewer{To Reviewer eESp \& iAim:}
\issue{On batch sizes and memory requirements} 
We commit to explicitly state the batch size employed (20,6,3) for each input resolution (128x256, 256x512, 512x1024) in section 4.1 in the revised version of the manuscript.  

For comparison, proposals employing the same architecture e.g. IPNB employing a DeeplabV3 with a WideResNet-38 backbone,  employs batch sizes of 28, 20 and 12 for resolutions of 512, 640 and 872 respectively. Meanwhile we employ less than a $9^{th}$ of their batch size, thus, allowing us to train with less memory budget. Experimental exploration with their code with a restricted batch size of 3, lead to a drop in performance of over 4 points in mIoU (79 to 75).
%
%However, as we are memory restricted, we can only theorize that our results will improve if larger batch sizes were employed when training using the proposed method. 
Preliminary experiments in our framework with smaller input resolutions resulted in almost a 15\% drop in performance (75 to 66 mIoU) when the batch size was reduced from 20 to 3 in the 128x256 input resolution. Similar results have been reported with  up to a 300\%  increase in performance when the batch size is increased from 2 to 8 [17,40].

Regarding the missing information in Table 3, authors of [31] and [20] do not explicitly state the memory resources required for training. However, we commit to include in the revised version a conservative estimation based on the batch size, architecture and input resolution information provided by the authors. %Explicitly, [20] employs batch sizes of 32 and 24 for resolutions of 128x128 and 256x256 respectively. Given the trained architecture, a minimum of 12GB GPU memory would be needed to fit such batch size (ignoring the computational overhead included by their sampling model ). Regarding [31], authors straightly refer to [3] for the omitted setup parameters, whereas [3] states that a minimum batch size of 8 is needed to train their method. Therefore, a minimum of 24GB would be needed for a 256x512 resolution whereas a minimum of 96GB would be required for a 512x1024 resolution. 

\toreviewer{To Reviewer jkGV:}
\issue{Improvements.} We would like to remark that \textbf{our code, trained models and logs will be published upon acceptance}. However, to provide further justification, we conduct a simple experiment quantifying the label noise included by our method compared to the (default) nearest neighbors (NN) one. Table \ref{tab:noise} measures the label changes when down-sampling the original resolution images using different factors and then up-sampling back to the original resolution employing the Cityscapes dataset. Note that the largest benefit is obtained when half resolution images are used, as our method conserves the full entropy of the label distribution whereas NN only conserves one out of four labels. The effect is critical for sampling patches in which several labels coexist and specially affect small objects, resulting in \textbf{more than a 10\% of labels corruption}. This training noise is compensated in the literature by enlarging the batch size [17,40] and/or the introduction of neighbourhood losses [2, 19] which aim at weighting down the classification loss in the edges of semantic structures. Note also that this NN-inherent label noise is present even when training using full resolution, as random resize crop is a common data augmentation strategy in semantic segmentation. This table and one discriminating the effect per class will be included in the supplementary material.

\begin{table}[]
    \centering
    \begin{tabular}{c c c }
         Method& Scale & $\mu$, min, max\\ \midrule
         NN & $\frac{1}{8}$ &12.60$\pm$ 3.00 ($\mu = 12.60, min= 9.05, max=15.55$) \\
         Ours & & 1.96$\pm$ 0.27 $\mu = 1.96, min= 1.69, max=2.25$\\\hdashline
         NN & $\frac{1}{4}$ &11.44$\pm$ 3.82 $\mu = 11.44, min= 7.62, max=14.33$\\
         Ours & &0.69$\pm$ 0.1 $\mu = 0.69, min= 0.59, max=0.79$ \\\hdashline
         NN & $\frac{1}{2}$ &11.08$\pm$ ¿? $\mu = 11.08, min= 0.00, max=13.89$\\
         Ours & &0.06$\pm$ 0.01$\mu = 0.06, min= 0.00, max=0.07$ \\\bottomrule
    \end{tabular}
    \caption{Mean $\pm$ standard deviation of label changes percentage. Measured by by down-sampling and up-sampling back images of the Cityscapes dataset. Statistics obtained from  applying the standard random scale protocol during 10 epochs for different scale factors.}
    \label{tab:noise_2}
\end{table}

\toreviewer{To Reviewer iAim:}
\issue{On the presentation of experimental performances} We acknowledge that the distinction between Tables 4 and 5, frameworks trained at full and under full resolution, can seem arbitrary. Therefore, we commit to unify tables 3, 4 and 5 into a single table comparing the proposals trained with the same architecture (DeeplabV3 and HRNetV2). Having the first half of the table with efficient proposals and the second half with the rest of the proposals.

%Due to the different implications the common sampling strategy brings to different objectives tables were selected to target each field. Table 3 aims to illustrate the benefits of the sampling strategy for smaller input resolutions and efficient proposals. However, Tables 4 and 5 can send a confusing message. Due to Table 4 comparing proposals trained under full resolution and table 5 comparing proposals trained at full resolution. Table 5 goal was to illustrate that with a worse performing architecture (HRNet), we manage to compete with better performing architectures (SegNext). Therefore, Table 5 will be changed (or removed) to include proposals trained with full resolution.

\toreviewer{To Reviewer jkGV \& iAim:}
\issue{Technical implementation} 
Following the valuable comments of the reviewers we will modify Eq 5 and Eq 6 to represent a scalar value.

\toreviewer{To Reviewer jkGV:}
\issue{Ablation study} 
First of all we would like to remark that \textbf{the loss employed is not a contribution of the paper}. As stated in the paper, formally both equations are equivalent due to $\hat{\mathbf{y}}$ being a constant value. However, both losses have different gradients due to the numerical computation and the base of the logarithms. Typically, KL is employed in statistical analysis which more commonly employs natural logarithm. Meanwhile, CE is employed in machine learning, which typically employs base 2 logarithm. This slight discrepancy, makes each of them scale different with respect to the soft-label $\mathbf{\hat{y}}$. Nevertheless, we acknowledge that this discrepancy is anecdotal in the context of the paper, where the main target of analysis is the impact of multi-labelled (MC) pixels information in the learning. Therefore, we commit to extend the section D of the Suplementary Material illustrating the gradient discrepancy.


\begin{equation}
    -\sum_{h,w} \sum_c  \hat{\mathbf{y}}^c_{h,w}log(G(\mathbf{x})^c_{h,w})
   
   
   \text{Equiation 5 of the paper for cross entropy loss}
\end{equation}

\begin{equation}
    \sum_{h,w} \sum_c  \hat{\mathbf{y}}^c_{h,w}log\left(\frac{\hat{\mathbf{y}}^c_{h,w}}{G(\mathbf{x})^c_{h,w}}\right) 

    
    \text{Equiation 6 of the paper for kullback-leibler  loss}
\end{equation}

\begin{equation}
\begin{split}
     KL(\hat{\mathbf{y}},G(\mathbf{x}))& =\sum_{h,w} \sum_c  \hat{\mathbf{y}}^c_{h,w}log\left(\frac{\hat{\mathbf{y}}^c_{h,w}}{G(\mathbf{x})^c_{h,w}}\right)  \\
     &=- \sum_{h,w} \sum_c  \hat{\mathbf{y}}^c_{h,w}log(G(\mathbf{x})^c_{h,w}) - \hat{\mathbf{y}}^c_{h,w}log(\hat{\mathbf{y}}^c_{h,w}) \\
     &=- \sum_{h,w} \sum_c  \hat{\mathbf{y}}^c_{h,w}log(G(\mathbf{x})^c_{h,w}) +\\
     &  \hspace{7mm}\sum_{h,w} \sum_c \hat{\mathbf{y}}^c_{h,w}log(\hat{\mathbf{y}}^c_{h,w}) \\
     &= CE(\hat{\mathbf{y}},G(\mathbf{x}))  - H(\hat{\mathbf{y}})
\end{split}
\end{equation}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Gradients.pdf}
    \caption{Gradient discrepancy comparison with respect to the entropy of the semantic label $\mathbf{\hat{y}}$. Gradients are compared for one epoch with the Cityscapes dataset images as training, with an identical network initialization and a common seed for dataset loader (both runs were shown the same images in the same order).}
    \label{fig:Gradients}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Mono_vs_Multi.png}
    \caption{Loss statistics of last epoch of training for a model trained with the CE loss and the KL loss. Model trained with the Cityscapes dataset}
    \label{fig:my_label} 
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{PerPixel.png}
    \caption{Loss statistics of first and last epochs of training for each of the multi class pixels types with the employment of CE loss and the KL loss. Model trained on the Cityscapes dataset}
    \label{fig:my_label} 
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{PerPixel_includingMono.png}
    \caption{Loss statistics of first and last epochs of training for each of the pixels types with the employment of CE loss and the KL loss. Model trained on the Cityscapes dataset}
    \label{fig:my_label} 
\end{figure}

\begin{table}[tp]
    \centering
    \resizebox{1\linewidth}{!}{%
    \begin{tabular}{c c c c c}
         Name&Architecture  & Resolution & GPU & mIoU \\ \hline
         %Espnetv2\cite{mehta2018espnetv2} & Espnetv2 &$512\times1024$& 12GB & 66.2\\
         %DSRLSS\cite{Wang_2020_CVPR}&Espnetv2 &$512\times1024$& 24GB* & 66.9\\
         %Mscfnet\cite{DBLP:journals/corr/abs-2103-13044}&Mscfnet & $512\times1024$ & 12GB  &71.9\\
         LDNSB\cite{9008795}& DeeplabV3+  & $128\times128$ & 12GB*&  62 \\
         DSRLSS\cite{Wang_2020_CVPR}&DeeplabV3+ & $256\times512$& 24GB* & 59.2\\
         LDNSB\cite{9008795} &DeeplabV3+ & $256\times256$ & 12GB*&65\\\hdashline
         Ours& DeeplabV3+& $128\times256$ & 12GB&72.66 \\
         Ours& DeeplabV3+ & $256\times512$& 12GB& 77.66\\
         %RealtimeSS\cite{HAO2021104269} & $512\times1024$ & 12GB & 73.7\\\hline
         Ours & HRNetv2 & $128\times256$ & 12GB&75.28\\
         Ours &HRNetv2  &$256\times512$ & 12GB&\textbf{81.95} \\\midrule
         DSRLSS\cite{Wang_2020_CVPR}&DeeplabV3+ &$512\times1024$& 96GB* & 73.4\\
         IPBN\cite{rotabulo2017place} & DeeplabV3+ & $872\times872$ & $(24\times 10)$GB & 79.4\\
         DeeplabV3+\cite{deeplabv3plus2018}& DeeplabV3+ & $513\times513$ & $(24\times 50)$GB&79.55\\
         ProgressiveSS\cite{m_Huynh-etal-CVPR21}&HRNetv2&$128\times256$& $(16\times 8)$GB &67.57\\
         Rethinking\cite{zhou2022rethinking}&HRNetv2& $768\times768$ & $(32\times 8)$GB& 81.1\\
         HRNetv2\cite{9052469}& HRNetv2&$1024\times2048$ & $(32\times 4)$GB& 81.6\\
         OCR\cite{YuanCW20}& HRNetv2 &$769\times769$ & $(24\times 10)$GB & 81.8\\
         DHSS\cite{li2022deep}&HRNetv2& $512\times1024$& $(40\times 4)$GB& 83.4\\\hdashline
         Ours & DeeplabV3+ & $512\times1024$ & 24GB &81.26\\
         %Ours &HRNetv2  &$256\times512$ & 24GB&82.01 \\
         Ours& HRNetv2  & $512\times1024$ & 24GB & \textbf{84.37}\\\hline
    \end{tabular}}
    
    \caption{ Performance and training requirements comparison of different state of the art semantic segmentation frameworks on the Cityscapes validation set. GPU stands for the amount of GPU memory required for training. Reference methods' performances are as reported in their papers. When memory requirements are not provided '*', we provide an estimated minimum requirement based on batch size and architecture.}
    \label{tab:SOTA_COMP_CS_LW}
\end{table}



\begin{table}[tp]
    \centering
    \resizebox{1\linewidth}{!}{%
    \begin{tabular}{c c c c c}
         Name&Architecture  & Resolution & GPU & mIoU \\ \hline
         IPBN\cite{rotabulo2017place} & DeeplabV3+ & $872\times872$ & $(24\times 10)$GB & 79.4\\
         DeeplabV3+\cite{deeplabv3plus2018}& DeeplabV3+ & $513\times513$ & $(24\times 50)$GB&79.55\\
         ProgressiveSS\cite{m_Huynh-etal-CVPR21}&HRNetv2&$128\times256$& $(16\times 8)$GB &67.57\\
         Rethinking\cite{zhou2022rethinking}&HRNetv2& $768\times768$ & $(32\times 8)$GB& 81.1\\
         HRNetv2\cite{9052469}& HRNetv2&$1024\times2048$ & $(32\times 4)$GB& 81.6\\
         OCR\cite{YuanCW20}& HRNetv2 &$769\times769$ & $(24\times 10)$GB & 81.8\\
         DHSS\cite{li2022deep}&HRNetv2& $512\times1024$& $(40\times 4)$GB& 83.4\\
         SegNext[10]*&SegNext& $1024\times2048$& $(32\times 8)$GB& 83.9\\\hdashline
         Ours & DeeplabV3+ & $512\times1024$ & 24GB &81.26\\
         %Ours &HRNetv2  &$256\times512$ & 24GB&82.01 \\
         Ours& HRNetv2  & $512\times1024$ & 24GB & \textbf{84.37}\\\hline
    \end{tabular}}
    
    \caption{ Performance and training requirements comparison of different state of the art semantic segmentation frameworks on the Cityscapes validation set. GPU stands for the amount of GPU memory required for training. Reference methods' performances are as reported in their papers. }
    \label{tab:SOTA_COMP_CS_LW}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{c c c c}
         Proposal& BS & Resolution & Performance  \\\toprule
         IPBN* & 28& 512 &77.8\\
         IPBN & 3 & 512 & 75.1\\
         Baseline & 3 & 512 & 76.1\\\hdashline
         Ours & 3 & 128 & 66\\
         Ours & 20 & 128 & 75\\
         Ours & 3 & 256 & 77 \\
         Ours & 6 & 256 & 81\\
         Ours & 12 & 256 & 82\\\bottomrule
         \end{tabular}
    \caption{Ablation study on the batch size for different resolutions and proposals. Reported results are marked with a '*'}
    \label{tab:my_label}
\end{table}
%%%%%%%%% REFERENCES
%{\small
%\bibliographystyle{ieee_fullname}
%\bibliography{egbib}
%}

\FloatBarrier
\myemptypage
\myemptypage\myemptypage\myemptypage

PIXEL LEVEL LOSSES


$CE(\hat{\mathbf{y}}_{h,w},G(\mathbf{x})_{h,w}) & = -\sum_c \hat{\mathbf{y}}^c_{h,w}log(G(\mathbf{x})^c_{h,w})$, and Eq. 6 for $KL(\hat{\mathbf{y}}_{h,w},G(\mathbf{x})_{h,w})& = \sum_c  \hat{\mathbf{y}}^c_{h,w}log\left(\frac{\hat{\mathbf{y}}^c_{h,w}}{G(\mathbf{x})^c_{h,w}}\right)$, and also moving the relationship between both losses:
\begin{equation}
\resizebox{\columnwidth}{!}{%

\begin{split}
     KL(\hat{\mathbf{y}}_{h,w},G(\mathbf{x})_{h,w})&=- \sum_c  \hat{\mathbf{y}}^c_{h,w}log(G(\mathbf{x})^c_{h,w}) - \hat{\mathbf{y}}^c_{h,w}log(\hat{\mathbf{y}}^c_{h,w}) \\
     &=- \sum_c  \hat{\mathbf{y}}^c_{h,w}log(G(\mathbf{x})^c_{h,w}) + \sum_c \hat{\mathbf{y}}^c_{h,w}log(\hat{\mathbf{y}}^c_{h,w}) \\
     &=  CE(\hat{\mathbf{y}}_{h,w},G(\mathbf{x})_{h,w})  - H(\hat{\mathbf{y}}_{h,w}),
\end{split}
}
\end{equation}
Illustrating how for each pixel in an image there is a different weighting down factor.



Batch LEVEL LOSSES


$L_{CE} = \sum_b CE(\hat{\mathbf{y}}^b,G(\mathbf{x})^b) = \sum_b -\sum_c \hat{\mathbf{y}}^{c,b}_{h,w}log(G(\mathbf{x})^{c,b}_{h,w})$, and Eq. 6 for $L_{KL} = \sum_b KL(\hat{\mathbf{y}}^b,G(\mathbf{x}^b)) = \sum_b\sum_{h,w}\sum_c  \hat{\mathbf{y}}^{c,b}_{h,w}log\left(\frac{\hat{\mathbf{y}}^{c,b}_{h,w}}{G(\mathbf{x})^{c,b}_{h,w}}\right)$, and also moving the relationship between both losses:
\begin{equation}
\resizebox{\columnwidth}{!}{%
\begin{split}
     KL(\hat{\mathbf{y}^b}_{h,w},G(\mathbf{x}^b)_{h,w})&=-\sum_b\sum_{h,w} \sum_c  \hat{\mathbf{y}}^{c,b}_{h,w}log(G(\mathbf{x})^{c,b}_{h,w}) - \hat{\mathbf{y}}^{c,b}_{h,w}log(\hat{\mathbf{y}}^{c,b}_{h,w}) \\
     &=- \sum_b\sum_{h,w}\sum_c  \hat{\mathbf{y}}^{c,b}_{h,w}log(G(\mathbf{x})^{c,b}_{h,w}) + \sum_b\sum_{h,w}\sum_c \hat{\mathbf{y}}^{c,b}_{h,w}log(\hat{\mathbf{y}}^{c,b}_{h,w}) \\
     &= \hspace{4mm} \sum_b CE(\hat{\mathbf{y}}^b,G(\mathbf{x}^b))  - H(\hat{\mathbf{y}}^b),
\end{split}
}
\end{equation}
Illustrating how for each image in the batch the weighting down factor is variable.



%%% PRUEBA MEV

\textbf{R3.W2, R2.W1} ask for \textcolor{red}{changing the formulation of the loss functions}. We propose to change Eq. 5 for
% \begin{equation}
%     CE(\hat{\mathbf{y}},G(\mathbf{x})) & = -\sum_{h,w} \sum_c  \hat{\mathbf{y}}^c_{h,w}log(G(\mathbf{x})^c_{h,w})$
% \end{equation}
% , and equation 6 by:
% \begin{equation}
%     KL(\hat{\mathbf{y}},G(\mathbf{x}))& =\sum_{h,w} \sum_c  \hat{\mathbf{y}}^c_{h,w}log\left(\frac{\hat{\mathbf{y}}^c_{h,w}}{G(\mathbf{x})^c_{h,w}}\right)
% \end{equation}
$\mathcal{L}_{CE} =  \sum_b CE(\hat{\mathbf{y}}^b,G(\mathbf{x})^b)$, with $ CE(\hat{\mathbf{y}}^b,G(\mathbf{x})^b) =  \sum_{h,w} CE(\hat{\mathbf{y}}_{h,w},G(\mathbf{x})_{h,w})$, being the cross-entropy loss for each image $b$ in the batch and $ CE(\hat{\mathbf{y}}^b_{h,w},G(\mathbf{x})^b_{h,w}) = -\sum_c \hat{\mathbf{y}}^{b,c}_{h,w}log(G(\mathbf{x})^{b,c}_{h,w})$ the cross-entropy per pixel image.

Similarly, we propose to change equation 6 for $\mathcal{L}_{KL} =  \sum_b KL(\hat{\mathbf{y}}^b,G(\mathbf{x})^b)$, with $ KL(\hat{\mathbf{y}}^b,G(\mathbf{x})^b) =  \sum_{h,w} KL(\hat{\mathbf{y}}^b_{h,w},G(\mathbf{x})^b_{h,w})$, being the KL-divergence between the prediction and the ground-truth of each image $b$ in the batch and $KL(\hat{\mathbf{y}}^b_{h,w},G(\mathbf{x})^b_{h,w}) = \sum_c  \hat{\mathbf{y}}^{b,c}_{h,w}log\left(\frac{\hat{\mathbf{y}}^{b,c}_{h,w}}{G(\mathbf{x})^{b,c}_{h,w}}\right)$ that of each image pixel. Furthermore, we will move the relationship between both losses:

\begin{equation}
\resizebox{\columnwidth}{!}{%
\begin{split}
     \mathcal{L}_{KL}&=-\sum_b\sum_{h,w} \sum_c  \hat{\mathbf{y}}^{c,b}_{h,w}log(G(\mathbf{x})^{c,b}_{h,w}) - \hat{\mathbf{y}}^{c,b}_{h,w}log(\hat{\mathbf{y}}^{c,b}_{h,w}) \\
     &=- \sum_b\sum_{h,w}\sum_c  \hat{\mathbf{y}}^{c,b}_{h,w}log(G(\mathbf{x})^{c,b}_{h,w}) + \sum_b\sum_{h,w}\sum_c \hat{\mathbf{y}}^{c,b}_{h,w}log(\hat{\mathbf{y}}^{c,b}_{h,w}) \\
     &= \hspace{4mm} \mathcal{L}_{CE}  - \sum_b\sum_{h,w} H(\hat{\mathbf{y}}^b_{h,w}),
\end{split}
}
\end{equation}
to the supplementary material, as it is surplus for the paper.

\textbf{R2.W2} may find this new formulation clearer to assess that \textcolor{red}{the optimization of both losses is not equivalent}. The gradient is computed on the aggregated loss per batch. Unlike $\mathcal{L}_{CE}$, the $\mathcal{L}_{KL}$ allows each pixel in the batch to differently contribute to the loss, as its loss penalty term, $H(\hat{\mathbf{y}}^b_{h,w})$, depends on its soft label distribution. Thus, only the loss of single-label pixels (zero entropy distribution) equally contribute for CE and KL. This was partially discussed in section D of the supplementary material, explaining  why the margin gets narrower for larger resolutions (i.e., less non-zero entropy multi-label pixels), and is sustained also by the loss statistics depicted in Figure \ref{fig:KL-vs-CE_loss}, which will be added to the supplementary material.


%%% PRUEBA 2 MEV

\textbf{R3.W2, R2.W1} ask for \textcolor{red}{changing the formulation of the loss functions}. We propose to change Eq. 5 for

$\mathcal{L}_{CE} =  \sum_{b,h,w} CE(\hat{\mathbf{y}}^b_{h,w},G(\mathbf{x})^b_{h,w})$, with $ CE(\hat{\mathbf{y}}^b_{h,w},G(\mathbf{x})^b_{h,w}) = -\sum_c \hat{\mathbf{y}}^{b,c}_{h,w}log(G(\mathbf{x})^{b,c}_{h,w})$ the cross-entropy for each pixel of each image $b$ in the batch.

Similarly, we propose to change Eq. 6 for $\mathcal{L}_{KL} =  \sum_{b,h,w} KL(\hat{\mathbf{y}}^b_{h,w},G(\mathbf{x})^b_{h,w})$, with $KL(\hat{\mathbf{y}}^b_{h,w},G(\mathbf{x})^b_{h,w}) = \sum_c  \hat{\mathbf{y}}^{b,c}_{h,w}log\left(\frac{\hat{\mathbf{y}}^{b,c}_{h,w}}{G(\mathbf{x})^{b,c}_{h,w}}\right)$. 
Moving the to the supplementary material\textemdash as a surplus, the relationship between both:
\begin{equation}
\resizebox{\columnwidth}{!}{%
\begin{split}
     \mathcal{L}_{KL}&=-\sum_{b,h,w} \sum_c  \hat{\mathbf{y}}^{c,b}_{h,w}log(G(\mathbf{x})^{c,b}_{h,w}) - \hat{\mathbf{y}}^{c,b}_{h,w}log(\hat{\mathbf{y}}^{c,b}_{h,w}) \\
     &=- \sum_{b,h,w} \sum_c  \hat{\mathbf{y}}^{c,b}_{h,w}log(G(\mathbf{x})^{c,b}_{h,w}) + \sum_{b,h,w} \sum_c \hat{\mathbf{y}}^{c,b}_{h,w}log(\hat{\mathbf{y}}^{c,b}_{h,w}) \\
     &= \hspace{4mm} \mathcal{L}_{CE}  - \sum_{b,h,w} H(\hat{\mathbf{y}}^b_{h,w}),
\end{split}
}
\end{equation}

\textbf{R2.W2} may find this new formulation clearer to assess that \textcolor{red}{the optimization of both losses is not equivalent}. The gradient is computed on the aggregated loss per batch. Unlike the $\mathcal{L}_{CE}$, the $\mathcal{L}_{KL}$ allows each pixel in the batch to differently contribute to the loss, as its loss penalty term, $H(\hat{\mathbf{y}}^b_{h,w})$, depends on its soft label distribution. Thus, only the loss of single-label pixels (zero entropy distribution) equally contribute for $\mathcal{L}_{CE}$ and $\mathcal{L}_{KL}$. This was partially discussed in section D of the supplementary material, explaining  why the margin gets narrower for larger resolutions (i.e., less non-zero entropy multi-label pixels), and is sustained also by the loss statistics depicted in Figure \ref{fig:KL-vs-CE_loss}, which will be added to the supplementary material.

